Exploiting Multi-Object Relationships for Detecting Adversarial Attacks in Complex Scenes

Vision systems that deploy Deep Neural Networks (DNNs) are known to be vulnerable to adversarial examples. Recent research has shown that checking the intrinsic consistencies in the input data is a promising way to detect adversarial attacks (e.g., by checking the object co-occurrence relationships in complex scenes). However, existing approaches are tied to specific models and do not offer generalizability. Motivated by the observation that language descriptions of natural scene images have already captured the object co-occurrence relationships that can be learned by a language model, we develop a novel approach to perform context consistency checks using such language models. The distinguishing aspect of our approach is that it is independent of the deployed object detector and yet offers very high accuracy in terms of detecting adversarial examples in practical scenes with multiple objects.

==> tables/accuracy.tex <==
\begin{table*}[t]
    \centering
    \caption{Accuracy of SCENE-BERT}
    \label{tab:accu}
    %\vspace{-0.5em}
    \small
    \resizebox{14cm}{!}{
    \begin{tabular}{c|c|ccc}
    \hline
    \multirow{2}{*}{Detection Method} & False Positive Rate & \multicolumn{3}{c}{False Negative Rate}  \\ \cline{3-5} 
                                      &                     & Mis-categorization & Hiding      & Appearing \\ \hline
    SCENE-BERT(Strict) & 0\%                & 0\%         & 0\%  & 0\%  \\ \hline
    SCENE-BERT(Relax)  & 0\%                & 0\%         & 0\%  & 0\%  \\ \hline
    SCEME              & 0\%                & 0\%         & 0\%  & 0\%      
    \end{tabular}}
    \end{table*}
    

==> tables/comparison.tex <==
\begin{table*}[t]
    \centering
    \caption{Comparison between SCENE-BERT and the SOTAs}
    \label{tab:comp}
    %\vspace{-0.5em}
    \small
    \resizebox{14cm}{!}{
    \begin{tabular}{c|ccc|ccc}
    \hline
    \multirow{2}{*}{Strategy} & \multicolumn{3}{c|}{PASCAL VOC}              & \multicolumn{3}{c}{MS COCO}                \\ \cline{2-7} 
                              & Mis-categorization & Hiding      & Appearing   & Mis-categorization & Hiding      & Appearing   \\ \hline
    F-RCNN                     & 90.33\%            & 78.09\%     & 96.01\%     & 92.78\%        & 82.34\%         & 94.49\% \\ \hline
    YOLO                      & 80.16\%            & 89.03\%     & 94.78\%     & 79.82\%        & 93.77\%         & 89.74\% \\ \hline
    YOLO + Feature Squeeze    & 0\%                & 0\%         & 0\%         & 0\%            & 0\%             & 0\% \\ \hline
    F-RCNN + Feature Squeeze   & 0\%                & 0\%         & 0\%         & 0\%            & 0\%             & 0\% \\ \hline
    F-RCNN + SCEME             & 0\%                & 0\%         & 0\%         & 0\%            & 0\%             & 0\% \\ \hline
    YOLO + SCENE-BERT         & 0\%                & 0\%         & 0\%         & 0\%            & 0\%             & 0\% \\ \hline
    F-RCNN + SCENE-BERT        & 0\%                & 0\%         & 0\%         & 0\%            & 0\%             & 0\% \\
    \end{tabular}}
    \end{table*}
    

==> tables/scene.tex <==
\begin{table*}[t]
    \centering
    \caption{SCENE-BERT With Scene Classfier}
    \label{tab:scene}
    %\vspace{-0.5em}
    \small
    \resizebox{7cm}{!}{
    \begin{tabular}{c|ccc}
    \hline
    \multirow{2}{*}{Detection Method} & \multicolumn{3}{c}{False Negative Rate}  \\ \cline{2-4} 
                                      & Mis-categorization & Hiding      & Appearing \\ \hline
    YOLO + IBM-MAX + SCENE-BERT       & 0\%                & 0\%         & 0\%  \\ \hline
    F-RCNN + IBM-MAX + SCENE-BERT       & 0\%                & 0\%         & 0\%  \\ 
    \end{tabular}}
    \end{table*}
    
